X-IL: Exploring the Design Space of Imitation Learning Policies

Designing modern imitation learning (IL) policies requires making numerous decisions, including the selection of feature encoding, architecture, policy representation, and more. As the field rapidly advances, the range of available options continues to grow, creating a vast and largely unexplored design space for IL policies. In this work, we present X-IL, an accessible open-source framework designed to systematically explore this design space. The framework's modular design enables seamless swapping of policy components, such as backbones (e.g., Transformer, Mamba, xLSTM) and policy optimization techniques (e.g., Score-matching, Flow-matching). This flexibility facilitates comprehensive experimentation and has led to the discovery of novel policy configurations that outperform existing methods on recent robot learning benchmarks. Our experiments demonstrate not only significant performance gains but also provide valuable insights into the strengths and weaknesses of various design choices. This study serves as both a practical reference for practitioners and a foundation for guiding future research in imitation learning.

==> figures/blocks_ablation/blocks_ablation.tex <==
\begin{figure}[t!]
        \centering
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/blocks_ablation/beso_mamba.pdf}
                \includegraphics[width=0.48\textwidth]{figures/blocks_ablation/beso_xlstm.pdf}
            \end{minipage}
        \caption[ ]
        {Ablation study for encoder-decoder structures.}
        \label{fig:blocks_ablation}
\end{figure}


==> results/tables/architecture_ablations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{BESO}
& \textbf{LIBERO-10}(20\%)
& \textbf{LIBERO-10}(100\%)
% & \textbf{OpenDrawer}
& \textbf{TurnOnStove}
& \textbf{CoffeeServeMug}
\\ 
\midrule
Dec-Transformer
& $40.5 \scriptstyle \pm 2.2$
& $79.3 \scriptstyle \pm 0.9$
& $30.7 \scriptstyle \pm 3.8$
& $18.0 \scriptstyle \pm 4.3$
\\
Dec-Mamba
& $46.3 \scriptstyle \pm 3.4$
& \boldsymbol{$85.2 \scriptstyle \pm 1.9$}
& $28.0 \scriptstyle \pm 3.3$
& $20.7 \scriptstyle \pm 3.4$
\\
Dec-xLSTM
& \boldsymbol{$51.8 \scriptstyle \pm 3.6$}
& $84.1 \scriptstyle \pm 2.6$
& \boldsymbol{$34.7 \scriptstyle \pm 2.5$}
& \boldsymbol{$30.7 \scriptstyle \pm 5.2$}
\\
\midrule
CrossAttn-Transformer
& $56.0$
& $42.0$
& $32.0$
& $48.0$
\\
ADaln-Transformer
& $56.0$
& $42.0$
& $32.0$
& $48.0$
\\
ADaln-Mamba
& $56.0$
& $42.0$
& $32.0$
& $48.0$
\\
ADaln-xLSTM
& $56.0$
& $42.0$
& $32.0$
& $48.0$
\\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
% \vskip -0.15in
    \caption{Comparison on BESO with different architectures. Notice that here we train models only on the TurnOnStove and CoffeeServeMug tasks, so the results could be different from Table \ref{table:main_results_2d}
    }
    % \vspace{-0.2cm}
\label{table:ablation_architecture}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/inference_time_architecture.tex <==
\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l|l}
\hline
\textbf{} & \textbf{Transformer} & \textbf{MAMBA } & \textbf{xLSTM} \\ \hline
Dec-Image (ms)          & $34.17\scriptstyle \pm 0.63$ & $45.37\scriptstyle \pm 0.75$  & $75.60\scriptstyle \pm 1.52$  \\ 
Encdec-Image (ms)            & $47.78\scriptstyle \pm 1.44$ & $52.90\scriptstyle \pm 1.05$ & $76.58\scriptstyle \pm 1.08$  \\ \hline
Dec-Point Cloud (ms)         & $40.27\scriptstyle \pm 0.16$ & $45.77\scriptstyle \pm 0.35$ & $399.65\scriptstyle \pm 8.59$  \\
Encdec-Point Cloud (ms)       & $43.36\scriptstyle \pm 0.24$ & $48.49.77\scriptstyle \pm 0.33$ & $181.07\scriptstyle \pm 2.20$  \\ \hline
\end{tabular}
}
\caption{Inference Speed comparison using BESO policy head, 16 sampling steps; number of decoder layers(transformer, mamba, xlstm):  10/14/12;  number of enc-dec layers: 4+6/6+8/4+8}
\label{tab:sample_table}
\end{table}

==> results/tables/inference_time_diffusion.tex <==
% \begin{table}[h!]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{p{16mm}|l|l|l|l|l}
% \hline
% \textbf{Sample Steps} & \textbf{1} & \textbf{4} & \textbf{8} & \textbf{12} & \textbf{16}\\ \hline
% DDPM (ms)          & $4.03\scriptstyle \pm 0.01$ & $10.34\scriptstyle \pm 0.17$   & $18.53 \scriptstyle \pm 0.30$   & $27.41\scriptstyle \pm 0.64$   & $35.65 \scriptstyle \pm 0.68$\\
% BESO (ms)          & $4.03\scriptstyle \pm 0.01$ & $10.34\scriptstyle \pm 0.17$   & $18.53 \scriptstyle \pm 0.30$   & $27.41\scriptstyle \pm 0.64$   & $35.65 \scriptstyle \pm 0.68$\\
% FM (ms)            & $3.84\scriptstyle \pm 0.10$ & $9.96\scriptstyle \pm 0.15$ & $18.00\scriptstyle \pm 0.38$ & $26.33\scriptstyle \pm 0.62$ & $34.17\scriptstyle \pm 0.63$ \\ \hline
% \end{tabular}
% }
% \caption{Comparison of DDPM, BESO, and Flow Matching across different sampling steps}
% \label{tab:sample_table}
% \end{table}

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{16mm}|l|l|l}
\hline
\textbf{Sample Steps} & DDPM (ms) & BESO(ms) & FM(ms) \\ \hline
\textbf{1}  & $4.91\scriptstyle \pm 0.05$ & $4.98\scriptstyle \pm 0.09$  & $5.02\scriptstyle \pm 0.03$ \\
\textbf{4}  & $14.62\scriptstyle \pm 0.28$ &$14.91\scriptstyle \pm 0.29$ & $14.63\scriptstyle \pm 0.34$\\
\textbf{8}  & $27.39\scriptstyle \pm 0.48$ &$28.00\scriptstyle \pm 0.68$ & $27.65\scriptstyle \pm 0.66$\\
\textbf{12} & $40.40\scriptstyle \pm 0.80$ &$40.43\scriptstyle \pm 0.75$ & $40.11\scriptstyle \pm 0.74$\\
\textbf{16} &$53.39\scriptstyle \pm 1.21$ &$53.78\scriptstyle \pm 1.17$ & $52.96\scriptstyle \pm 1.08$\\ \hline
\end{tabular}
}
\caption{Comparison of DDPM, BESO, and Flow Matching across different sampling steps}
\label{tab:sample_table}
\end{table}

==> results/tables/parameters.tex <==
\begin{table}[hbtp]
\centering
\resizebox{.95\textwidth}{!}{  
\renewcommand{\arraystretch}{1.2}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\small
\begin{tabular}{l|c|c|c|c}
	\toprule 
         Method & Layers & Params & Inference time (RGB) & Inference time (PC)\\
	\midrule
        Transformer \\
        \midrule
        Dec    & 4 & 27.0M &  \\
               & 6 & 29.1M &  \\
               & 8 & 31.2M &  \\
               & 10 & 33.3M & \\
        EncDec & 4+6 & 34.9M &  \\
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        Mamba \\
        \midrule
        Dec    & 6 & 27.1M &  \\
               & 8 & 28.5M &  \\
               & 10 & 29.9M & \\
               & 12 & 31.3M & \\
               & 14 & 32.7M & \\
               & 16 & 34.1M & \\
        EncDec & 4+8 & 34.5M &  \\
               & 6+8 & 35.9M & \\
	\midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        XLSTM \\
        \midrule
        Dec    & 10 & 27.1M &  \\
               & 16 & 29.6M &  \\
               & 20 & 31.3M & \\
        EncDec &  &  &  \\
        \bottomrule
\end{tabular}

}
\vspace{0.1cm}

\caption{Inference Time Comparison, we compare different architectures using flow matching policy for both visual inputs and point cloud inputs}\label{parameter}
\vskip -0.15in
\end{table}
